TBV Radar SLAM -- trust but verify loop candidates

Robust SLAM in large-scale environments requires fault resilience and awareness at multiple stages, from sensing and odometry estimation to loop closure. In this work, we present TBV (Trust But Verify) Radar SLAM, a method for radar SLAM that introspectively verifies loop closure candidates. TBV Radar SLAM achieves a high correct-loop-retrieval rate by combining multiple place-recognition techniques: tightly coupled place similarity and odometry uncertainty search, creating loop descriptors from origin-shifted scans, and delaying loop selection until after verification. Robustness to false constraints is achieved by carefully verifying and selecting the most likely ones from multiple loop constraints. Importantly, the verification and selection are carried out after registration when additional sources of loop evidence can easily be computed. We integrate our loop retrieval and verification method with a fault-resilient odometry pipeline within a pose graph framework. By evaluating on public benchmarks we found that TBV Radar SLAM achieves 65% lower error than the previous state of the art. We also show that it's generalizing across environments without needing to change any parameters.

==> Journal/figures/tables/TabMulranATE.tex <==

\begin{table*}[t!]
\centering
\vspace{0.2cm}
 \begin{adjustbox}{width=\textwidth}
\begin{tabular}{ll|l|l|lllllllll|ll}
           %            & & & & & \multicolumn{3}{l}{\textbf{Mulran Sequence}}    & \\
\cline{2-14}
&\textbf{Type/Modality}& \textbf{Method}  & \textbf{Evaluation} & \texttt{KAIST01} & \texttt{KAIST02} & \texttt{KAIST03} & \texttt{DCC01} & \texttt{DCC02} & \texttt{DCC03} & \texttt{RIV.01} & \texttt{RIV.02} & \texttt{RIV.03} & Mean\\
\cline{2-14}
\ldelim\{{7.5}{30pt}[ATE]&&&&&&&&&&&&&&  \rdelim\}{7.5}{30pt}[ATE]
\\[-2ex]
&SLAM/Lidar & SuMa Full~\cite{behley2018rss}  &~\cite{hongSLAM_IJRR}  &  {38.70} & {31.90} & {46.00} & {13.50} & {17.80} & {29.60} & {-} & {-} & {-} & {22.90}  \\
&Odometry/Lidar&KISS-ICP (odometry)~\cite{vizzo2022arxiv}  &  &  {17.40} & {17.40} & {17.40} & {15.16 } & {15.16} & {15.16} & {49.02} & {49.02} & {49.02} & {27.2}\\
\cline{2-14}
\\[-2ex]
&Odometry/Radar&CFEAR-3~\cite{cfear_journal} (odometry used) & & 7.53 & 7.58 & 12.21 & 6.39 & 3.67 & 5.40 & 6.45 & 3.87 & 19.44 & 8.06\\
%\rowcolor{Gray} 
&\mycc  \textbf{SLAM/Radar} &\mycc RadarSLAM Full~\cite{hongSLAM_ARXIV}  &\mycc ~\cite{hongSLAM_IJRR} &\mycc {6.90} &\mycc {6.00} &\mycc {4.20} &\mycc {12.90} &\mycc {9.90} &\mycc {3.90} &\mycc {9.00} &\mycc {7.00} &\mycc {10.70} &\mycc {7.80} \\
&\mycc  \textbf{SLAM/Radar} &\mycc MAROAM Full~\cite{MAROAM}  &\mycc ~\cite{MAROAM} &\mycc {-} &\mycc {-} &\mycc {-} &\mycc {-} &\mycc {5.81} &\mycc {-} &\mycc {-} &\mycc {4.85} &\mycc {-} &\mycc {-} \\

%\rowcolor{Gray}
%&\mycc \textbf{SLAM/Radar} &\mycc TBV SLAM-1 (ours) &\mycc &\mycc 2.29 &\mycc 2.36 &\mycc \textbf{1.43} &\mycc 5.54 &\mycc 3.8  &\mycc 3.45 &\mycc 2.82 &\mycc 2.59 &\mycc 1.69 &\mycc 2.88 \\
%\rowcolor{Gray}  
&\mycc \textbf{SLAM/Radar} &\mycc TBV SLAM-T.8-dyn-cov (ours) &\mycc &\mycc  \underbar{1.71} &\mycc      \underbar{1.42} &\mycc      \underbar{1.52} &\mycc    \textbf{5.41} &\mycc    \textbf{3.29} &\mycc    \textbf{2.61} &\mycc  \underbar{2.66} &\mycc          \underbar{2.49} &\mycc \underbar{2.52} &\mycc   \underbar{2.63}  \\
&\mycc \textbf{SLAM/Radar} &\mycc TBV SLAM-T.8-cov (ours) &\mycc &\mycc \textbf{1.66} &\mycc \textbf{1.39} &\mycc \textbf{1.50}  &\mycc \underbar{5.44} &\mycc \underbar{3.32} &\mycc \underbar{2.66} &\mycc \textbf{2.61} &\mycc \textbf{2.36} &\mycc \textbf{1.48} &\mycc \textbf{2.49} \\
%\textbf{TBV SLAM-7} (ours) & & \textbf{1.65} & \textbf{1.39} & \textbf{1.50} & \textbf{5.44}  & \textbf{3.33} & \textbf{2.67} & \textbf{2.61} & \textbf{2.37} & \textbf{1.52} & \textbf{2.50}\\
\cline{2-14}\\[-2ex]
\cline{2-14} 
%PhaRaO-Full~\cite{9197231} &  &  -/12.8 & -/12.8 & -/12.8 & -/13.26 & -/13.26 & -/13.26 & -/31.8 & -/31.8 & -/31.8 & -/19.3\\
%CFEAR-3  & 0.0595 & 0.06/15.17 & 0.06/19.56 & 0.06/39.47 & 0.08/10.10 & 0.04/7.63 & 0.05/8.16 & 0.06/26.70 & 0.05/41.16 & 0.04/24.01 &  5.77/21.33 & {-} & {-} \\
%CFEAR-3-10  & 0.0595 & 0.06/9.98 & 0.06/5.60 & 0.06/10.70 & 0.07/7.13 & 0.04/4.69 & 0.04/6.00 & 0.06/12.27 & 0.05/19.03 & 0.04/18.60 &  0.05/10.44 & {-} & {-} \\
%CFEAR-3-50  & 0.0595 & 0.06/14.42 & 0.06/13.91 & 0.06/33.52 & 0.08/9.60 & 0.04/5.82 & 0.05/8.56 & 0.06/22.51 & 0.06/44.24 & 0.05/22.08 & 5.80/19.41 & {-} & {-} \\
\ldelim\{{6.5}{30pt}[Drift]&&&&&&&&&&&&&&  \rdelim\}{6.5}{30pt}[Drift]\\[-2ex]
&SLAM/Lidar & SuMa Full~\cite{behley2018rss}  &   & 2.9/0.8 & 2.64/0.6 & 2.17/0.6 & 2.71/0.4 & 4.07/0.9 & 2.14/0.6 & 1.66/0.6$^P$ & 1.49/0.5$^P$ & 1.65/0.4$^P$ & 2.38/0.5 & \\
&Odometry/Lidar & KISS-ICP (odometry)~\cite{vizzo2022arxiv}  &  &  {2.28/0.68} & {2.28/0.68} & {2.28/0.68} & {2.34/0.64} & {2.34/0.64 } & {2.34/0.64 } & {2.89/0.64} & {2.89/0.64} & {2.89/0.64} & {2.5/0.65} &\\
\cline{2-14} \\[-2ex]
%LOAM~\cite{loam} &  & 3.31/0.99 & 2.74/0.87 & 7.56/0.85 & 3.36/0.92 & 2.85/0.79 & 2.47/0.82 & 6.47/0.96 & 6.14/0.96 & 3.93/1.02 & 4.21/0.92
%&Odometry/Radar&RadarSLAM-odometry~\cite{hongSLAM_ARXIV}  & ~\cite{hongSLAM_IJRR}  &   2.13/0.7 & 2.07/0.6 & 1.99/0.5 & 2.70/0.5 & 1.90/0.4 & 1.64/0.4 &  2.04/0.5 & 1.51/0.5& 1.71/0.5 & 1.97/0.5&
&Odometry/Radar & CFEAR-3-s50~\cite{cfear_journal}  & ~\cite{cfear_journal}  &  \underbar{1.48}/0.65 & \underbar{1.51}/0.63 & \underbar{1.59}/0.75 & \underbar{2.09}/0.55 & \underbar{1.38}/0.47 & \underbar{1.26}/0.47 & 1.62/\underbar{0.62} & \underbar{1.35}/0.52 & 
\underbar{1.19/0.37} & \underbar{1.50}/0.56 &
  
\\
&Odometry/Radar&CFEAR-3~\cite{cfear_journal} (odometry used)  & & 1.59/0.66 & 1.62/0.66 & 1.73/0.78 & 2.28/0.54 & 1.49/0.46 & 1.47/0.48 & \underbar{1.59}/0.63 & 1.39/\underbar{0.51} & 1.41/0.40 &  1.62/0.57 &
\\
%CFEAR-3-s50  & 0.0595 & \textbf{1.48/0.65} & \textbf{1.51}/0.63 & \textbf{1.59}/0.75 & \textbf{2.09}/0.55 & \textbf{1.38}/0.47 & \textbf{1.26}/0.47 & \textbf{1.62}/0.62 & \textbf{1.35}/0.52 & \textbf{1.19/0.37} & \textbf{1.50}/0.56 & - & -
%\rowcolor{Gray} 
&\mycc   \textbf{SLAM/Radar} &\mycc RadarSLAM-Full~\cite{hongSLAM_ARXIV}  &\mycc ~\cite{hongSLAM_IJRR} &\mycc  1.75/\underbar{0.5} &\mycc 1.76/\underbar{0.4} &\mycc 1.72/\underbar{0.4} &\mycc 2.39/\underbar{0.4} &\mycc 1.90/\underbar{0.4} &\mycc 1.56/\textbf{0.2} &\mycc  3.40/0.9 &\mycc 1.79/\textbf{0.3} &\mycc 1.95/0.5 &\mycc 2.02/\underbar{0.4} \\
%\rowcolor{Gray}
%&\mycc  \textbf{SLAM/Radar} &\mycc  TBV SLAM-1 (ours) &\mycc  &\mycc 1.01/0.29 &\mycc 1.06/0.31 &\mycc 1.08/0.35 &\mycc 2.02/0.28 &\mycc 1.36/0.25 &\mycc 1.16/0.23 &\mycc \textbf{1.23/0.35} &\mycc 1.10/0.29 &\mycc 1.01/0.18 &\mycc 1.22/0.28\\
%\rowcolor{Gray} 
%&\mycc  \textbf{SLAM/Radar} &\mycc  TBV SLAM-8-dyn (ours) &\mycc  &\mycc \textbf{1.01/0.30} &\mycc 1.01/0.29 &\mycc  1.05/0.31 &\mycc  1.09/0.35 &\mycc  2.01/0.28 &\mycc  1.34/0.25 &\mycc  1.15/0.23 &\mycc  1.29/0.37     &\mycc  1.09/0.30     &\mycc  1.09/0.22     & &\mycc 1.24/0.29 \\
&\mycc  \textbf{SLAM/Radar} &\mycc  TBV SLAM-T.8 (ours) &\mycc  &\mycc \textbf{1.01/0.30} &\mycc \textbf{1.03/0.30} &\mycc \textbf{1.08/0.35} &\mycc \textbf{2.01/0.27} &\mycc \textbf{1.35/0.25} &\mycc \textbf{1.14}/\underbar{0.22} &\mycc \textbf{1.25/0.35} &\mycc \textbf{1.09/0.30} &\mycc \textbf{0.99/0.18} &\mycc \textbf{1.22/0.28} \\
\cline{2-14} 
% \textbf{TBV SLAM-7} (ours) &  & \textbf{0.99/0.29} & \textbf{1.03/0.30} & \textbf{1.08/0.35} & \textbf{2.01/0.28} & \textbf{1.35/0.25} & \textbf{1.15/0.22} & \textbf{1.25/0.35} & \textbf{1.08/0.30} & \textbf{0.99/0.18} &  \textbf{1.21/0.28} & \\
\end{tabular}
  \end{adjustbox}
  %\vspace{-0.2cm}
\caption{ Top: Absolute Trajectory error (ATE), Bottom: Drift (\% translation error / deg/$100$~m) on the \texttt{MulRan} dataset~\cite{gskim_2020_mulran}. 
\changed{Methods for Radar SLAM are shaded.
The best and second best radar results are marked in \textbf{bold}/\underbar{underlined}.}
}
\label{tab:TabMulRanATE}
%\vspace{-0.cm}
\end{table*}

==> Journal/figures/tables/TabOxfordATE.tex <==
\definecolor{Gray}{gray}{0.9}
\begin{table*}[b!]
%\vspace{-0.2cm}
\centering
  \begin{adjustbox}{width=\textwidth}
  %\vspace{-0.4cm}
\begin{tabular}{ll|l|l|llllllll|ll}
%\setlength{\textfloatsep}{0.5cm}
    %          & & & & & \multicolumn{2}{l}{\textbf{Oxford Sequence}}    &  \\
\cline{2-13}
& \textbf{Type/modality} & \textbf{Method} & \textbf{Evaluation} &  \texttt{10-12-32}$^\text{Training}$ & \texttt{16-13-09} & \texttt{17-13-26} & \texttt{18-14-14} & \texttt{18-15-20} & \texttt{10-11-46} & \texttt{16-11-53} & \texttt{18-14-46} & Mean\\
%ORB-SLAM2     & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1    & 1         \\
\cline{2-13}
\ldelim\{{6.5}{30pt}[ATE]&&&&&&&&&&&&&  \rdelim\}{6.5}{30pt}[ATE]
%&&&&&&&&&&&&\\
%\rdelim\}{7}{30pt}[ATE]
\\[-2ex]
%& SLAM/Lidar & SuMa (Lidar - SLAM)~\cite{behley2018rss}  & ~\cite{hongSLAM_ARXIV }& - & - & - & - & -  & -        & -        & -        &  -  \\
& SLAM/camera & ORB-SLAM2~\cite{7946260} &~\cite{hongSLAM_ARXIV } & 7.96 & 7.59 & 7.61 &  24.63 & 12.17 & 7.30      & 3.54       &  9.72      &  10.07 \\
\cline{2-13}\\[-2ex]
%& Odometry/Radar & RadarSLAM-odometry~\cite{hongSLAM_IJRR} & ~\cite{hongSLAM_ARXIV} &  $2.32/0.7$        & $2.62/0.7$        & $ 2.27/0.6$        & $2.29/0.7$        & $2.25/0.7$        & $2.16/0.6$        & $2.49/0.7$        & $2.12/0.6$        & $2.32/0.7$\\
%CFEAR-3-s50 (ours) &  & $0.0438$ & 6.0 & \textbf{1.05/0.34} & \textbf{1.08/0.34} & \textbf{1.07/0.36} & \textbf{1.11/0.37} & \textbf{1.03/0.37} & \textbf{1.05/0.36} & \textbf{1.18/0.36} & \textbf{1.11/0.36} &  \textbf{1.09/0.36} &  - & -  \\
& Odometry/Radar & CFEAR-3 (odometry used) & & 7.29 &      23.32 &      15.58 &      20.95 &      20.02 &      16.87 &      15.47 &      28.58 &  18.51\\
\cline{2-13} \\[-2ex]
%  \rowcolor{Gray}
&  \mycc \textbf{SLAM/Radar} &  \mycc RadarSLAM-Full~\cite{hongSLAM_IJRR} &\mycc ~\cite{hongSLAM_ARXIV} &\mycc 9.59        &\mycc 11.18       &\mycc 5.84       &\mycc 21.21        &\mycc 7.74       &\mycc 13.78        &\mycc 7.14        &\mycc 6.01       &\mycc 10.31\\
&  \mycc \textbf{SLAM/Radar} &  \mycc MAROAM~\cite{MAROAM} &\mycc {From author} &\mycc 13.76        &\mycc 6.95       &\mycc 8.36       &\mycc 10.34        &\mycc 10.96       &\mycc 12.42        &\mycc 12.51        &\mycc  7.71       &\mycc 10.38\\


 %\rowcolor{Gray}
%&\mycc \textbf{SLAM/Radar} &\mycc TBV SLAM-1 (ours) &\mycc &\mycc 6.12 &\mycc 3.96 &\mycc 3.81 &\mycc 4.95 &\mycc 4.42 &\mycc 5.03 &\mycc 4.2  &\mycc 4.93 &\mycc 4.68 \\
%\rowcolor{Gray}

&\mycc  \textbf{SLAM/Radar} &\mycc \tbv{}-dyn-cov-T.8 (ours)  &\mycc &\mycc \underbar{4.22} &\mycc \underbar{4.30}  &\mycc \textbf{3.37} &\mycc \underbar{4.04} &\mycc \underbar{4.27} &\mycc \underbar{3.38} &\mycc \underbar{4.98} &\mycc \textbf{4.27} &\mycc \underbar{4.10}  \\
&\mycc  \textbf{SLAM/Radar} &\mycc \tbv{}-T.8 (ours)  &\mycc &\mycc \textbf{4.07} &\mycc \textbf{4.04} &\mycc \underbar{3.58} &\mycc \textbf{3.79} &\mycc \textbf{3.83} &\mycc       \textbf{3.14} &\mycc \textbf{4.39} &\mycc \underbar{4.33} &\mycc \textbf{3.90} \\
%DRIF
\cline{2-13}\\[-2ex]
\cline{2-13} 
\ldelim\{{6.5}{30pt}[Drift]&&&&&&&&&&&&&  \rdelim\}{6.5}{30pt}[Drift]
\\[-2ex]
%& Odometry/Vision & Visual Odometry  ~\cite{Churchill2012ExperienceBN} & ~\cite{barnes_masking_2020} & -  & - & -        & -        & -        & -        & -        & -        &   $ 3.980/1.0$\\
%ORB-SLAM2     & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1    & 1         \\
& SLAM/Lidar & SuMa (Lidar - SLAM)~\cite{behley2018rss}  & ~\cite{hongSLAM_ARXIV} & $1.1/0.3^p$ & $1.2$/$0.4^p$ & $1.1/0.3^p$ & $0.9/0.1^p$ & $1.0/0.2^p$  & $1.1/0.3^p$        & $0.9/0.3^p$        & $1.0/0.1^p$        &  $1.03/0.3^p$\\
\cline{2-13} \\[-2ex]
%& Odometry/Radar & RadarSLAM-odometry~\cite{hongSLAM_IJRR} & ~\cite{hongSLAM_ARXIV} & $2.32/0.7$        & $2.62/0.7$        & $ 2.27/0.6$        & $2.29/0.7$        & $2.25/0.7$        & $2.16/0.6$        & $2.49/0.7$        & $2.12/0.6$        & $2.32/0.7$\\
&   \textbf{Odometry/Radar} & CFEAR-3-S50~\cite{cfear_journal} (Offline) &  ~\cite{cfear_journal} & \textbf{1.05/0.34} & \textbf{1.08/0.34} & \underbar{1.07/0.36} & \textbf{1.11/0.37} & \textbf{1.03}/\underbar{0.37} & \textbf{1.05}/\underbar{0.36} & \textbf{1.18/0.36} & \underbar{1.11}/\textbf{0.36} &  \textbf{1.09}/\textbf{0.36}\\

& Odometry/Radar & CFEAR-3 (odometry used) & & 1.20/0.36  & 1.24/0.40  & 1.23/0.39  & 1.35/0.42  & 1.24/0.41  & 1.22/0.39  & 1.39/0.40  & 1.39/0.44  & 1.28/0.40\\
\cline{2-13}
\\[-2ex]
 %\rowcolor{Gray}
 &\mycc  \textbf{SLAM/Radar} &\mycc RadarSLAM-Full~\cite{hongSLAM_IJRR} &\mycc ~\cite{hongSLAM_ARXIV} &\mycc $1.98/0.6$        &\mycc $1.48/0.5$        &\mycc $1.71/0.5$        &\mycc $2.22/0.7$        &\mycc $1.77/0.6$        &\mycc $1.96/0.7$        &\mycc $1.81/0.6$        &\mycc $1.68/0.5$        &\mycc $1.83/0.6$\\
 &
 %
  \mycc  \textbf{SLAM/Radar} &\mycc MAROAM-Full~\cite{MAROAM} &\mycc ~\cite{MAROAM} &\mycc $1.63/0.46$        &\mycc $1.83/0.56$        &\mycc $1.49/0.47$        &\mycc $1.54/0.47$        &\mycc $1.61/0.50$        &\mycc $1.55/0.53$        &\mycc $1.78/0.54$        &\mycc $1.55/0.50$        &\mycc $1.62/0.50$\\

%\rowcolor{Gray}
%&\mycc   \textbf{SLAM/Radar} &\mycc TBV SLAM-1 (ours) &\mycc   &\mycc 1.19/0.35  &\mycc 1.17/0.36  &\mycc 1.11/0.37  &\mycc 1.18/0.39  &\mycc 1.14/0.37  &\mycc 1.23/0.37  &\mycc 1.34/0.37  &\mycc 1.17/0.39  &\mycc 1.19/0.37 \\

%\rowcolor{Gray}
&\mycc  \textbf{SLAM/Radar} &\mycc \tbv{}-T.8 (ours) &\mycc   &\mycc \underbar{1.17/0.35}  &\mycc \underbar{1.15/0.35}  &\mycc \textbf{1.06/0.35}  &\mycc \underbar{1.12}/\textbf{0.37}  &\mycc \underbar{1.09}/\textbf{0.36}  &\mycc \underbar{1.18}/\textbf{0.35}  &\mycc \underbar{1.32}/\textbf{0.36}  &\mycc \textbf{1.10/0.36}  &\mycc \underbar{1.15}/\textbf{0.36} \\
\end{tabular}
\end{adjustbox}
\vspace{-0.2cm}
\caption{ Top: Absolute Trajectory error (ATE) [m], Bottom: Drift (\% translation error / deg/$100$~m) on the \texttt{Oxford Radar RobotCar} dataset~\cite{RadarRobotCarDatasetICRA2020}. Methods marked with p finished prematurely. Methods for Radar SLAM  are shaded.
\changed{The best and second best radar results are marked in \textbf{bold}/\underbar{underlined}.}
}\label{tab:TabOxfordATE}
\vspace{-0.1cm}
\end{table*}

==> Journal/figures/tables/backup/TabMulranDrift.tex <==
\begin{table*}[h!]
\centering
 \begin{adjustbox}{width=\textwidth}
\begin{tabular}{l|l|lllllllll|l}
              & & & \multicolumn{1}{l}{\textbf{Sequence}}\\
\textbf{Method}  & \textbf{Evaluation} & KAIST01 & KAIST02 & KAIST03 & DCC01 & DCC02 & DCC03 & RIV01 & RIV02 & RIV03 & Mean\\
\hline \\
SuMa Full~\cite{behley2018rss}  &   & 2.9/0.8 & 2.64/0.6 & 2.17/0.6 & 2.71/0.4 & 4.07/0.9 & 2.14/0.6 & 1.66/0.6 & 1.49/0.5 & 1.65/0.4 & 2.38/0.5 \\
KISS-ICP (odometry)~\cite{vizzo2022arxiv}  &  &  {2.28/0.68} & {2.28/0.68} & {2.28/0.68} & {2.34/0.64} & {2.34/0.64 } & {2.34/0.64 } & {2.89/0.64} & {2.89/0.64} & {2.89/0.64} & {2.5/0.65}\\
\hline\\
%LOAM~\cite{loam} &  & 3.31/0.99 & 2.74/0.87 & 7.56/0.85 & 3.36/0.92 & 2.85/0.79 & 2.47/0.82 & 6.47/0.96 & 6.14/0.96 & 3.93/1.02 & 4.21/0.92
RadarSLAM-Full~\cite{hongSLAM_ARXIV}  & ~\cite{hongSLAM_IJRR} &  1.75/0.5 & 1.76/0.4 & 1.72/0.4 & 2.39/0.4 & 1.90/0.4 & 1.56/0.2 &  3.40/0.9 & 1.79/0.3 & 1.95/0.5 & 2.02/0.4 \\
\hline\\
RadarSLAM-odometry~\cite{hongSLAM_ARXIV}  & ~\cite{hongSLAM_IJRR}  &   2.13/0.7 & 2.07/\textbf{0.6} & 1.99/\textbf{0.5} & 2.70/\textbf{0.5} & 1.90/\textbf{0.4} & 1.64/\textbf{0.4} &  2.04/\textbf{0.5} & 1.51/\textbf{0.5} & 1.71/0.5 & 1.97/\textbf{0.5}
\\
CFEAR-3 (our odometry)  & & 1.59/0.66 & 1.62/0.66 & 1.73/0.78 & 2.28/0.54 & 1.49/0.46 & 1.47/0.48 & 1.59/0.63 & 1.39/0.51 & 1.41/0.40 &  1.62/0.57
\\
%CFEAR-3-s50  & 0.0595 & \textbf{1.48/0.65} & \textbf{1.51}/0.63 & \textbf{1.59}/0.75 & \textbf{2.09}/0.55 & \textbf{1.38}/0.47 & \textbf{1.26}/0.47 & \textbf{1.62}/0.62 & \textbf{1.35}/0.52 & \textbf{1.19/0.37} & \textbf{1.50}/0.56 & - & -
TBV SLAM-1 (ours) &  & 1.01/0.29 & 1.06/0.31 & 1.08/0.35 & 2.02/0.28 & 1.36/0.25 & 1.16/0.23 & 1.23/0.35 & 1.10/0.29 & 1.01/0.18 & 1.22/0.28 \\
\textbf{TBV SLAM-7} (ours) &  & \textbf{0.99/0.29} & \textbf{1.03/0.30} & \textbf{1.08/0.35} & \textbf{2.01/0.28} & \textbf{1.35/0.25} & \textbf{1.15/0.22} & \textbf{1.25/0.35} & \textbf{1.08/0.30} & \textbf{0.99/0.18} &  \textbf{1.21/0.28} \\

\end{tabular}
  \end{adjustbox}
\caption{Drift evaluated over 9 sequences from the MulRan dataset~\cite{gskim-2020-mulran}. We compare various methods for lidar and radar odometry, and lidar/radar SLAM that additionally correct the trajectory. Results are given in (\% translation error / deg/$100$~m).}
\label{tab:TabMulranOdometry}
\vspace{-0.2cm}
\end{table*}

==> Journal/figures/tables/backup/TabOxfordDrift.tex <==
\begin{table*}[hb]
\vspace{0.2cm}
\centering
  \begin{adjustbox}{width=\textwidth}
\begin{tabular}{l|l|llllllll|l}
              & & & & \multicolumn{1}{l}{\textbf{Sequence}}    &  \\
\textbf{Method} & \textbf{Evaluation}   & 10-12-32$^{Training}$ & 16-13-09 & 17-13-26 & 18-14-14 & 18-15-20 & 10-11-46 & 16-11-53 & 18-14-46 & Mean  \\
\hline \\
Visual Odometry  ~\cite{Churchill2012ExperienceBN} & ~\cite{barnes_masking_2020} & -  & - & -        & -        & -        & -        & -        & -        &   $ 3.980/1.0$\\
%ORB-SLAM2     & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1    & 1         \\
SuMa (Lidar - SLAM)~\cite{behley2018rss}  & ~\cite{hong2020radarslam } & $1.1/0.3^p$ & $1.2$/$0.4^p$ & $1.1/0.3^p$ & $0.9/0.1^p$ & $1.0/0.2^p$  & $1.1/0.3^p$        & $0.9/0.3^p$        & $1.0/0.1^p$        &  $1.03/0.3^p$\\
\hline \\
RadarSLAM-odometry~\cite{hongSLAM_IJRR} & ~\cite{hongSLAM_ARXIV} & $2.32/0.7$        & $2.62/0.7$        & $ 2.27/0.6$        & $2.29/0.7$        & $2.25/0.7$        & $2.16/0.6$        & $2.49/0.7$        & $2.12/0.6$        & $2.32/0.7$\\

CFEAR-3 (our odometry) & & 1.23/0.36 & 1.25/0.39 & 1.25/0.40 & 1.34/0.41 & 1.26/0.41 & 1.26/0.39 & 1.42/0.39 & 1.42/0.44 & 1.31/0.40\\
\hline
\\
RadarSLAM-Full~\cite{hongSLAM_IJRR} & ~\cite{hongSLAM_ARXIV} &$1.98/0.6$        & $1.48/0.5$        & $1.71/0.5$        & $2.22/0.7$        & $1.77/0.6$        & $1.96/0.7$        & $1.81/0.6$        & $1.68/0.5$        & $1.83/0.6$\\

TBV SLAM-1 (ours) &   & 1.19/0.35  & 1.17/0.36  & 1.11/0.37  & 1.18/0.39  & 1.14/0.37  & 1.23/0.37  & 1.34/0.37  & 1.17/0.39  & 1.19/0.37 \\

\textbf{TBV SLAM-7} (ours) &   & \textbf{1.17/0.35}  & \textbf{1.15/0.35}  & \textbf{1.06/0.35}  & \textbf{1.12/0.37}  & \textbf{1.09/0.36}  & \textbf{1.18/0.35}  & \textbf{1.32/0.36}  & \textbf{1.11/0.36}  & \textbf{1.15/0.36} \\

\end{tabular}
\end{adjustbox}

\caption{Drift evaluated over 8 sequences from the Oxford dataset~\cite{RadarRobotCarDatasetICRA2020}. Results are given in (\% translation error / deg/$100$~m).
}\label{tab:TabOxfordOdometry}
\vspace{-0.2cm}
\end{table*}

==> Journal/figures/tables/backup/TabTimeEval.tex <==
\begin{table}[hb]
\vspace{-0.2cm}
\centering
  \begin{adjustbox}{width=\textwidth}
\begin{tabular}{lrrrrrrrrrrrr}

% & Pose graph optimization & Verify loop candidate & VerificationModel & VerifyByOdometry & Register & itrs & Apply contraints & Loop-full & Detect loop & gather statistics & VerifyByAlignment & Descriptor \\
\hline
       &   Optimization (992) &  Full verification (19)  &    Register(6) &  Loop-full(128) &   Detect loop (25) &   Descriptor(1)  & Odometry(37) & Add training data (236)\\
\hline
 time [ms]  & 992 & 19 & 6 & 128 & 25 & 1 & 37 & 236 \\

\hline
\end{tabular}
\end{adjustbox}

\caption{*Time eval...*
}\label{tab:TabTimeEval}
\vspace{-0.2cm}
\end{table}

==> Journal/figures/tex_figures/a.tex <==
\begin{figure*}[htb!]
	%\begin{adjustbox}{width=\textwidth}
	\centering
	\newcommand\figsize{0.1425\hsize}
	\newcommand\trimleft{1}
	\newcommand\trimright{0.4}
	\begin{center}
		\subfloat[T.1]{\includegraphics[trim={\trimleft cm 0cm  \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/1.pdf}\label{fig:1_qualitative}}
		\subfloat[T.2]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/2.pdf}\label{fig:2_qualitative}}
		\subfloat[T.3]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/3.pdf}\label{fig:3_qualitative}}
		\subfloat[T.4]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/4.pdf}\label{fig:4_qualitative}}
		\subfloat[T.5]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/5.pdf}\label{fig:5_qualitative}}
		\subfloat[T.6]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/6.pdf}\label{fig:6_qualitative}}
		\subfloat[T.8]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/7.pdf}\label{fig:7_qualitative}}
		\vspace{-0.2cm}
		\caption{Detected loops in the Oxford dataset using the methods in Sec.~\ref{sec:ablation}. All potential loops are colored and ordered according to success: red (dangerous failure --  False Positive), orange (safe failure -- False Negative), blue (safe failure -- False Negative), green (success -- True Positive).
		%Red: False loop detected. Orange: No loop detected (Suggested candidate is incorrect). 
		Blue-colored loops differ compared to orange in that the suggested candidates are actually correct, but no loop is predicted as likelihood doesn't exceed the decision boundary: ($y_{loop}^{q,c_k} < y_{th}$).
		 \label{fig:qualitative_loops}}
	\end{center}
	\vspace{-0.7cm}
	%\begin{adjustbox}{width=\textwidth}
\end{figure*}


==> Journal/figures/tex_figures/backup/kvarntorp_traj.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.99\columnwidth]{Journal/figures/evaluation/EstimatedTrajectory/Kvarntorp/kvarntorp_line20_alpha02.png}
    \caption{Kvarntorp sequence - TBV SLAM-7 (blue), CFEAR-3 (green)}
    \label{fig:kvarntorp_traj}
\end{figure}


==> Journal/figures/tex_figures/backup/oxford_loops.tex <==
\begin{figure*}[]
	%\begin{adjustbox}{width=\textwidth}
	\centering
	\newcommand\figsize{0.1425\hsize}
	\newcommand\trimleft{1}
	\newcommand\trimright{0.4}
	\begin{center}
		\subfloat[1]{\includegraphics[trim={\trimleft cm 0cm  \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/1.pdf}\label{fig:1_qualitative}}
		\subfloat[2]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/2.pdf}\label{fig:2_qualitative}}
		\subfloat[3]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/3.pdf}\label{fig:3_qualitative}}
		\subfloat[4]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/4.pdf}\label{fig:4_qualitative}}
		\subfloat[5]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/5.pdf}\label{fig:5_qualitative}}
		\subfloat[6]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/6.pdf}\label{fig:6_qualitative}}
		\subfloat[7]{\includegraphics[trim={\trimleft cm 0cm \trimright cm 0cm},clip,width=\figsize]{figures/evaluation/LoopClosure/qualitative/7.pdf}\label{fig:7_qualitative}}
		\caption{Detected loops in the Oxford dataset when using each of the methods in Sec.~\ref{sec:evaluated_methods}.
		Green: True loop detected, blue: true loop not detected (but with correct loop position), orange: true loop not detected (with incorrect loop position), red: false loop detected. \label{fig:qualitative_loops}}
	\end{center}
	%\vspace{-0.5cm}
	%\begin{adjustbox}{width=\textwidth}
\end{figure*}


==> Journal/figures/tex_figures/loop_closure_roc_mulran.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{Journal/figures/evaluation/LoopClosure/MulRan/mulran_ablation.pdf}
    \caption{Loop detection over 8 sequences in the MulRan dataset.}
    \label{fig:mulran_loop_closure_ablation}
\end{figure}


==> Journal/figures/tex_figures/loop_closure_roc_oxford.tex <==
q\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{Journal/figures/evaluation/LoopClosure/Oxford/oxford_ablation.pdf}
    \caption{Loop detection over 8 sequences in the Oxford dataset.}
    \label{fig:oxford_loop_closure_ablation}
\end{figure}


==> Journal/figures/tex_figures/volvo_kvarntorp.tex <==
\begin{figure}
    \centering
    	\subfloat[][VolvoCE - forest]{\includegraphics[trim={2cm 2cm 4cm 3cm},clip,width=.55\hsize]{Journal/figures/evaluation/EstimatedTrajectory/Volvo/volvo_line20_alpha02.png}\label{fig:volvo_qual}}\hfill \subfloat[][Kvarntorp - underground mine]{\includegraphics[trim={3cm 0cm 5cm 1cm},clip,width=.45\hsize]{Journal/figures/evaluation/EstimatedTrajectory/Kvarntorp/kvarntorp_line20_alpha02.png}\label{fig:kvarntorp_qual}}
    %\includegraphics[width=0.99\columnwidth]{Journal/figures/evaluation/EstimatedTrajectory/Volvo/volvo_line20_alpha02.png}
    \caption{SLAM within a forest and underground mine. TBV RADAR SLAM (blue),  CFEAR radar odometry (green).}
    \label{fig:volvo_kvarntorp}
    \vspace{-0.5cm}
\end{figure}


==> Journal/related_work.tex <==
Early methods for radar SLAM employ
filtering~\cite{6689216} and landmark graph SLAM~\cite{7795967}. We instead use pose-graph SLAM based on odometry and loop constraints obtained by registering scans.
Holder et al.~\cite{Holder_2019} proposed a pose graph SLAM based on automotive radar, using GLARE~\cite{GLARE_2014} for place recognition.
Their method uses gyroscope and wheel odometry to provide an initial alignment guess to \ac{ICP} for scan matching. 
Our method uses a pose graph back-end but relies solely on a spinning radar.

Recent progress in the development of spinning 2D radar has quickly inspired numerous works on radar odometry estimation~\cite{cen2018,cen2019,barnes_masking_2020,hong2020radarslam,barnes_under_2020,PhaRaO,kung2021normal,burnett_we_2021,burnett2021radar,hongSLAM_IJRR,adolfsson2021cfear,cfear_journal,what_goes_around,fmbm}, place recognition~\cite{barnes_under_2020,saftescu_kidnapped_2020,kradarplusplus,gadd_fool_me_once_place,gadd2020look,yin2021radar,RaLL},
topological localization~\cite{RaLL,kradarplusplus,replace_radar_lidar} localization in overhead imagery~\cite{RSLNET,self_sup_overhead} and SLAM~\cite{hong2020radarslam,hongSLAM_IJRR,MAROAM}.
Most similar to ours is the work by Wang et al.~\cite{MAROAM}, and the seminal work on radar SLAM by Hong et al.~\cite{hongSLAM_IJRR}. Hong et al.~\cite{hongSLAM_IJRR} estimates odometry and registers loop constraints using KLT tracker keypoints. For place recognition, they use adaptive thresholding to filter data, and M2DP~\cite{he2016m2dp} to compute and match descriptors. The trajectory is corrected using pose graph optimization. Our work brings a larger focus on the introspective verification of loop constraints.
Martini et al.~\cite{kradarplusplus} proposed a teach-and-repeat localization framework using a hierarchical approach. First, a place candidate is retrieved via nearest neighbor search within a learned metric space using the method by Saftescu et al.~\cite{saftescu_kidnapped_2020}.
Second, sensor pose is estimated (without the need for an initial guess) by finding and registering the (globally) optimal set of landmark matches as described by Cen et al.~\cite{cen2018}. 
Unlike ~\cite{kradarplusplus}, we use a fast local registration method, motivated by the access of an initial alignment guess from the place recognition module. However, we carefully verify registration success before accepting new loop constraints.

Verification of pose estimates is essential for safety.
E.g., such tests could have prevented a reported accident that occurred during an automated driving test~\cite{naoki_detection_of_loc}. 
Holder et al.~\cite{Holder_2019} verify the detected loop candidates using radar data by the condition that ICP residuals cannot exceed a set threshold. 
Rather than verifying loops as a final step (separated from loop detection), we unify loop retrieval and verification. 
Some works~\cite{kradarplusplus,8917111} use the landmark matching compatibility matrix~\cite{cen2018} to assess quality. Martini et al.~\cite{kradarplusplus} reject place candidates based on the quality score of the matrix. Aldera et al.~\cite{8917111} learn detection of pose estimate failures from features extracted from the eigenvectors of the compatibility matrix. Training labels are provided by an external ground truth system. We build on the method CorAl~\cite{ADOLFSSON2022104136} to detect false loop candidates or constraints.
In the lidar domain, Behley et al.~\cite{behley-2018-suma} accept only reappearing loop candidates that are consistent with odometry over multiple consecutive scans, we instead focus on verification using only individual scans.
Some methods attempt to measure how observations would constrain registration in the current scene; a low level of constraints in one direction suggests registration could be unstable. 
The measure has been used to predict the risk of registration failure~\cite{8462890,castellano-2022-alignability}, abstain from closing loops when risk is high~\cite{hongSLAM_IJRR}, or prioritize the inclusion of loop closures accordingly~\cite{denniston_darpa_loop_closure_prior}. We instead use odometry uncertainty as a prior, which we combine with additional loop evidence computed after registration.
Finally, a range of methods aims at verifying pose estimates by detecting point cloud misalignment~\cite{ADOLFSSON2022104136,learning_to_detect,naoki_detection_of_loc}. We fuse misalignment detection~\cite{ADOLFSSON2022104136} together with place similarity and odometry uncertainty to achieve robust unified loop detection and verification.  

%kdradar++, hierarchical 
%what can go wrong quality of compatabily matrix teach and repeat framework
%Lidar slam CT-ICP~\cite{ct_icp_slam} (elevation maps), suma~\cite{behley-2018-suma}. verifies loops via consistency over delta consecutive frames frames. We focus on verifying individual frames.
%LeGO LOAM SC ~\cite{lego_loam_sc}.
%cartographer~\cite{cartographer}
\label{sec:rw-radar} 

%Legeac radar SLAM paper~\cite{7795967,8813841} 

%or localization in a given map~\cite{7535489}. 

%Imaging lidar~\cite{robust2021shan}
%scan context~\cite{gkim-2018-iros,gskim-2021-tro}


